Fast Radio Bursts as Probes of Magnetic Fields in Galaxies at z < 0.5

We present a sample of nine Fast Radio Bursts (FRBs) from which we derive magnetic field strengths of the host galaxies represented by normal, $z<0.5$ star-forming galaxies with stellar masses $M_* \approx 10^8 -10^{10.5} M_\odot$. We find no correlation between the FRB rotation measure(RM) and redshift which indicates that the RM values are due mostly to the FRB host contribution. This assertion is further supported by strong correlations (Spearman test probabilities $P_S \simeq 0.05$) found between RM and the estimated host dispersion measure ($DM_{Host}$) and host-normalized galacto-centric offset (Spearman $r_S$ values equal to 0.64 and -0.52). For these nine galaxies, we estimate their magnetic field strengths projected along the sightline $B$ finding a low median value of $0.5 \mu G$. This implies the magnetic fields of our sample of hosts are weaker than those characteristic of the Solar neighborhood ($\approx 6 \mu G$), but relatively consistent with a lower limit on observed range of $2-10 \mu G$ for star-forming, disk galaxies, especially as we consider reversals in the B-field, and that we are only probing $B_{\parallel}$. We compare to RMs from simulated galaxies of the Auriga project -- magneto-hydrodynamic cosmological zoom simulations - and find that the simulations predict the observed values to within the $95\%$ CI. Upcoming FRB surveys will provide hundreds of new FRBs with high-precision localizations, rotation measures, and imaging follow-up to support further investigation on the magnetic fields of a diverse population of $z<1$ galaxies.

==> tab_rm.tex <==
\begin{deluxetable*}{cccccccccccccccc}
\tablewidth{0pc}
\tablecaption{Rotation Measures\label{tab:rm}}
\tabletypesize{\normalsize}
\tablehead{\colhead{FRB} & \colhead{RM} & \colhead{DM} 
\\ & ($rad m^{-2}$) & ($pc cm^{3}$) 
} 
\startdata 
20121102& 100000.000& 558.100\\ 
20180916& -114.600& 348.760\\ 
20180924A& 22.000& 362.160\\ 
20190102C& -105.000& 364.545\\ 
20190608B& 353.000& 340.050\\ 
20190711A& 9.000& 587.900\\ 
20191001A& 55.500& 507.900\\ 
20200120E& -29.800& 87.818\\ 
20201124A& -613.000& 411.000\\ 
\hline 
\enddata 
\end{deluxetable*} 

